Cross-View Completion Models are Zero-shot Correspondence Estimators

In this work, we explore new perspectives on cross-view completion learning by drawing an analogy to self-supervised correspondence learning. Through our analysis, we demonstrate that the cross-attention map within cross-view completion models captures correspondence more effectively than other correlations derived from encoder or decoder features. We verify the effectiveness of the cross-attention map by evaluating on both zero-shot matching and learning-based geometric matching and multi-frame depth estimation. Project page is available at https://cvlab-kaist.github.io/ZeroCo/.

==> Figure/tex/Teaser.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{example-image-duck}
    \caption{\textbf{Teaser.}} 
    \vspace{-10pt}
    
    \label{fig:main}
\end{figure}


==> Figure/tex/depth_qual.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{Figure/assets/fig5_mainqual_box.pdf}
    \caption{\textbf{Qualitative results of multi-frame depth estimation on KITTI~\cite{balntas2017hpatches}}
    }
    \vspace{-10pt}
    \label{fig:zeroshot_qual}
\end{figure*}

==> Figure/tex/main_architecture.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{Figure/assets/fig3_main_overview.pdf}
    \caption{\textbf{Main Architecture.}} 
    \vspace{-10pt}
    
    \label{fig:main}
\end{figure}


==> Figure/tex/zeroshot_qual.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{Figure/assets/fig4_zeroshot_qual.pdf}
    \vspace{-20pt}
    \caption{\textbf{Qualitative results of zero-shot matching on HPatches~\cite{balntas2017hpatches}}
    }
    \vspace{-10pt}
    \label{fig:zeroshot_qual}
\end{figure*}

==> Supple/Table/depth_ablation.tex <==
\begin{table}[t!]
\centering
\resizebox{\linewidth}{!}{

\begin{tabular}{c|c|c|ccc|c}
\toprule
Depth & \multicolumn{2}{c|}{Aggregation} & 
\multirow[c]{2}{*}{AbsRel$\downarrow$} &
\multirow[c]{2}{*}{SqRel$\downarrow$} &
\multirow[c]{2}{*}{RMSE$\downarrow$}  &
\multirow[c]{2}{*}{\textbf{$\delta_1$}$\uparrow$}\\
\cline{2-3}
head &  $\mathcal{F}_{attn}$ & $\mathcal{F}_{feat}$ &&&&\\
\midrule
\midrule
DPT  & \ding{55} & \ding{55} & 0.102 & 0.767 & 4.351 & 0.903 \\
Aggregator & \ding{51} & \ding{55} & 0.150 & 1.235 & 5.515& 0.808 \\
Aggregator  & \ding{55} & \ding{51} & 0.092 & 0.650 & 4.218 & 0.910\\
\midrule
Aggregator &\ding{51}&\ding{51}&  \textbf{0.090} & \textbf{0.637 }& \textbf{4.128} & \textbf{0.915}\\
\bottomrule
		\end{tabular}
	}
    \vspace{-5pt}
    \caption{\textbf{Ablation studies on the KITTI Dataset.}
    }
    \vspace{-10pt}
    \label{suptab:depth_abl}
\end{table}


==> Table/YFCC.tex <==
\begin{table}[t!]
\centering
\resizebox{\linewidth}{!}{

\begin{tabular}{l|ccc|ccc}
\toprule
\multirow[c]{2}{*}{ Methods } & \multicolumn{3}{c|}{AUC $\uparrow$} & \multicolumn{3}{c}{mAP $\uparrow$} \\
& @5$^\circ$ &
@10$^\circ$ &
@20$^\circ$ &
@5$^\circ$ &
@10$^\circ$ &
@20$^\circ$\\
\midrule \midrule
RANSAC-Flow~\cite{shen2020ransac} & - & - & - & 64.9 & 73.3 & 81.6 \\
PDC-Net~\cite{vaswani2017attention} & 35.7 & 55.8 & 72.3 & 65.2 & 74.2 & 82.4 \\
PDC-Net+~\cite{vaswani2017attention} & 37.5 & 58.1 & 74.5 & 67.4 & 76.6 & 84.6 \\
Pmatch~\cite{zhu2023pmatch} & 45.7 & 65.2 & 79.8 & 75.9 & 83.1 & 89.3 \\
DKM~\cite{edstedt2023dkm} & & & & & \\
RoMa~\cite{edstedt2024roma} & & & & \\
\midrule
\textbf{Ours} & & & & \\
\bottomrule
		\end{tabular}
	}
    \caption{\textbf{Two-view camera pose estimation on YFCC100m~\cite{thomee2016yfcc100m} dataset.}
    }
    \vspace{-5pt}
    \label{tab:megadepth}
\end{table}

==> Table/depth_cityscape.tex <==
\begin{table*}[t!]
\centering
\resizebox{0.85\textwidth}{!}{

\begin{tabular}{l|c|c|cccc|ccc}
\toprule
\multirow[c]{2}{*}{ Method } &
Additional &
Test &
\multirow[c]{2}{*}{AbsRel$\downarrow$} &
\multirow[c]{2}{*}{SqRel$\downarrow$} &
\multirow[c]{2}{*}{RMSE$\downarrow$} &
\multirow[c]{2}{*}{RMSElog$\downarrow$} &
\multirow[c]{2}{*}{$\delta_1$$\uparrow$} &
\multirow[c]{2}{*}{$\delta_2$$\uparrow$} &
\multirow[c]{2}{*}{$\delta_3$$\uparrow$}
\\
 &
network &
frames & &&&&&&
\\
\midrule
\midrule
Struct2Depth 2  ~\cite{casser2019unsupervised} & - & 1 & 0.145 & 1.737 & 7.280 & 0.205 & 0.813 & 0.942 & 0.976 \\
Monodepth2      ~\cite{godard2019digging}     & - & 1 & 0.129 & 1.569 & 6.876 & 0.187 & 0.849 & 0.957 & 0.983 \\
Videos in the Wild ~\cite{gordon2019depth}    & - & 1 & 0.127 & 1.330 & 6.960 & 0.195 & 0.830 & 0.947 & 0.981 \\
Li et al. \cite{li2021unsupervised}   & - & 1 & 0.119 & 1.290 & 6.980 & 0.190 & 0.846 & 0.952 & 0.982 \\
Struct2Depth 2  ~\cite{casser2019unsupervised} & $\mathcal{M}$, $\mathcal{F}$ & 3 (-1, 0, 1) & 0.151 & 2.492 & 7.024 & 0.202 & 0.826 & 0.937 & 0.972 \\
ManyDepth       ~\cite{watson2021temporal}   & $\mathcal{M}$  & 2 (-1, 0) & 0.114 & 1.193 & 6.223 & 0.170 & \underline{0.875} & 0.967 & \underline{0.989} \\
DynamicDepth$^\dagger$   ~\cite{feng2022disentangling} & $\mathcal{M}$, $\mathcal{S}$ & 2 (-1, 0) & \textbf{0.104} & \textbf{1.009} & \textbf{5.991} & \textbf{0.150} & \textbf{0.889} & \underline{0.972} & \textbf{0.991} \\
\midrule
% Baseline (ImageNet)             &&&&&&&& \\
% CroCo-Stereo (Baseline)                & 2 (-1, 0) &&&&&& \\
% \midrule
% \textbf{Ours (ImageNet)}                 &&&&&&&& \\
\textbf{Ours}                 & - & 2 (-1, 0) & \underline{0.105} & \underline{1.050} & \underline{6.117} & \underline{0.162} & \textbf{0.889} & \textbf{0.973} & \textbf{0.991} \\
\bottomrule
		\end{tabular}
	}
    \caption{\textbf{Depth estimation results on Cityscapes~\cite{cordts2016cityscapes}.} We compare our model with previous single- and multi-frame depth estimation networks. For our baseline, we adopted the CroCo-stereo architecture~\cite{weinzaepfel2023croco} and trained it using a self-supervised depth learning manner. The best is in \textbf{bold}, and the second best is \underline{underlined}. $\dagger$: our reproduced results from the official repository, $\mathcal{M}$: monocular depth~\citep{godard2019digging}, $\mathcal{S}$: segmentation, and $\mathcal{F}$: flow network.
    }
    \label{tab:cityscape}
\end{table*}

==> Table/megadepth_table.tex <==
\begin{table}[t!]
\centering
\resizebox{0.9\linewidth}{!}{

\begin{tabular}{l|ccc}
\toprule
Methods &
PCK-1$\uparrow$ &
PCK-3$\uparrow$ &
PCK-5$\uparrow$
\\
\midrule \midrule
RANSAC-Flow~\cite{shen2020ransac}  &  53.47 & 83.45 & 86.81 \\
GLU-Net-GOCor~\cite{truong2020gocor} & 57.77 & 78.61 & 82.24 \\
PDC-Net~\cite{vaswani2017attention} & 71.81 & 89.36 & 91.18 \\
PDC-Net+~\cite{vaswani2017attention} &  74.51 & 90.69 & 92.10 \\
Pmatch~\cite{zhu2023pmatch} &  79.83 & 95.18 & 96.52 \\
\midrule
\textbf{Ours} & 59.77 & 83.76 & 87.77 \\
\bottomrule
		\end{tabular}
	}
    \caption{\textbf{Dense geometric matching evaluation on MegaDepth~\cite{li2018megadepth} dataset.}
    }
    \vspace{-5pt}
    \label{tab:megadepth}
\end{table}

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


